Hydrodynamic forces on assemblies of non-spherical particles: orientation and voidage effects

This work provides a recipe for creating drag, lift and torque closures for static assemblies of axisymmetric, non-spherical particles. Apart from Reynolds number $Re$ and solids volume fraction $\epsilon_s$, we propose four additional parameters to characterize the flow through non-spherical particle assemblies. Two parameters consider the mutual orientations of particles (the orientation tensor eigenvalues $S_1$ and $S_2$) and two angles represent the flow direction (polar and azimuthal angles $\alpha$ and $\beta$). Interestingly, we observe that the hydrodynamic forces on the particles are independent of the mutual particle orientations. Rather, the most important parameter representing the particle configuration itself is the incident angle $\phi$ of the individual particles with respect to the incoming flow. Moreover, we observe that our earlier finding of sine-squared scaling of drag for isolated particles (Sanjeevi & Padding 2017) holds on average even for a multiparticle system in both the viscous and inertial regimes. Similarly, we observe that the average lift for a multiparticle system follows sine-cosine scaling, as is observed for isolated particles. Such findings are very helpful since the pressure drop of a packed bed or porous media can be computed just with the knowledge of orientation distribution of particles and their drag at $\phi=0^\circ$ and $\phi=90^\circ$ for a given $Re$ and $\epsilon_s$. With the identified dependent parameters, we propose drag, lift and torque closures for multiparticle systems.

==> pics/FD_comparison_eps0_3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{023}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{026}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{024}[tc][tc]{\matlabtextB $Re$}%
\psfrag{025}[bc][bc]{\matlabtextB $F_{D,\phi=90^\circ}$}%
\psfrag{027}[tc][tc]{\matlabtextB $Re$}%
\psfrag{028}[bc][bc]{\matlabtextB $F_{D,\phi=0^\circ}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $200$}%
\psfrag{002}[ct][ct]{\matlabtextC $400$}%
\psfrag{003}[ct][ct]{\matlabtextC $600$}%
\psfrag{004}[ct][ct]{\matlabtextC $800$}%
\psfrag{005}[ct][ct]{\matlabtextC $1000$}%
\psfrag{011}[ct][ct]{\matlabtextC $0$}%
\psfrag{012}[ct][ct]{\matlabtextC $200$}%
\psfrag{013}[ct][ct]{\matlabtextC $400$}%
\psfrag{014}[ct][ct]{\matlabtextC $600$}%
\psfrag{015}[ct][ct]{\matlabtextC $800$}%
\psfrag{016}[ct][ct]{\matlabtextC $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $50$}%
\psfrag{008}[rc][rc]{\matlabtextC $100$}%
\psfrag{009}[rc][rc]{\matlabtextC $150$}%
\psfrag{010}[rc][rc]{\matlabtextC $200$}%
\psfrag{017}[rc][rc]{\matlabtextC $0$}%
\psfrag{018}[rc][rc]{\matlabtextC $10$}%
\psfrag{019}[rc][rc]{\matlabtextC $20$}%
\psfrag{020}[rc][rc]{\matlabtextC $30$}%
\psfrag{021}[rc][rc]{\matlabtextC $40$}%
\psfrag{022}[rc][rc]{\matlabtextC $50$}%
%
%% </ytick>

==> pics/FD_comparison_eps0_5.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{026}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{029}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{027}[tc][tc]{\matlabtextB $Re$}%
\psfrag{028}[bc][bc]{\matlabtextB $F_{D,\phi=90^\circ}$}%
\psfrag{030}[tc][tc]{\matlabtextB $Re$}%
\psfrag{031}[bc][bc]{\matlabtextB $F_{D,\phi=0^\circ}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $200$}%
\psfrag{002}[ct][ct]{\matlabtextC $400$}%
\psfrag{003}[ct][ct]{\matlabtextC $600$}%
\psfrag{004}[ct][ct]{\matlabtextC $800$}%
\psfrag{005}[ct][ct]{\matlabtextC $1000$}%
\psfrag{012}[ct][ct]{\matlabtextC $0$}%
\psfrag{013}[ct][ct]{\matlabtextC $200$}%
\psfrag{014}[ct][ct]{\matlabtextC $400$}%
\psfrag{015}[ct][ct]{\matlabtextC $600$}%
\psfrag{016}[ct][ct]{\matlabtextC $800$}%
\psfrag{017}[ct][ct]{\matlabtextC $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $100$}%
\psfrag{008}[rc][rc]{\matlabtextC $200$}%
\psfrag{009}[rc][rc]{\matlabtextC $300$}%
\psfrag{010}[rc][rc]{\matlabtextC $400$}%
\psfrag{011}[rc][rc]{\matlabtextC $500$}%
\psfrag{018}[rc][rc]{\matlabtextC $0$}%
\psfrag{019}[rc][rc]{\matlabtextC $20$}%
\psfrag{020}[rc][rc]{\matlabtextC $40$}%
\psfrag{021}[rc][rc]{\matlabtextC $60$}%
\psfrag{022}[rc][rc]{\matlabtextC $80$}%
\psfrag{023}[rc][rc]{\matlabtextC $100$}%
\psfrag{024}[rc][rc]{\matlabtextC $120$}%
\psfrag{025}[rc][rc]{\matlabtextC $140$}%
%
%% </ytick>

==> pics/Fd_by_Fdisol.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{022}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{025}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{023}[tc][tc]{\matlabtextB $Re$}%
\psfrag{024}[bc][bc]{\matlabtextB $F_{D,\phi=90^\circ}(\epsilon_s)/F_{D,\phi=90^\circ}(\epsilon_s=0)$}%
\psfrag{026}[tc][tc]{\matlabtextB $Re$}%
\psfrag{027}[bc][bc]{\matlabtextB $F_{D,\phi=0^\circ}(\epsilon_s)/F_{D,\phi=0^\circ}(\epsilon_s=0)$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{-2}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{-1}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{0}$}%
\psfrag{003}[ct][ct]{\matlabtextC $10^{1}$}%
\psfrag{004}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{005}[ct][ct]{\matlabtextC $10^{3}$}%
\psfrag{011}[ct][ct]{\matlabtextC $10^{-2}$}%
\psfrag{012}[ct][ct]{\matlabtextC $10^{-1}$}%
\psfrag{013}[ct][ct]{\matlabtextC $10^{0}$}%
\psfrag{014}[ct][ct]{\matlabtextC $10^{1}$}%
\psfrag{015}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{016}[ct][ct]{\matlabtextC $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $5$}%
\psfrag{008}[rc][rc]{\matlabtextC $10$}%
\psfrag{009}[rc][rc]{\matlabtextC $15$}%
\psfrag{010}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $0$}%
\psfrag{018}[rc][rc]{\matlabtextC $5$}%
\psfrag{019}[rc][rc]{\matlabtextC $10$}%
\psfrag{020}[rc][rc]{\matlabtextC $15$}%
\psfrag{021}[rc][rc]{\matlabtextC $20$}%
%
%% </ytick>

==> pics/Fd_by_Fdisol_phicombined.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{010}[tc][tc]{\matlabtextA $\epsilon_s$}%
\psfrag{011}[bc][bc]{\matlabtextA $F_{D}(\epsilon_s)/F_{D}(\epsilon_s=0)$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{005}[ct][ct]{\matlabtextB $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0$}%
\psfrag{007}[rc][rc]{\matlabtextB $5$}%
\psfrag{008}[rc][rc]{\matlabtextB $10$}%
\psfrag{009}[rc][rc]{\matlabtextB $15$}%
%
%% </ytick>

==> pics/Fd_vs_Re.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{024}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{027}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{025}[tc][tc]{\matlabtextB $Re$}%
\psfrag{026}[bc][bc]{\matlabtextB $F_{D,\phi=90^\circ}$}%
\psfrag{028}[tc][tc]{\matlabtextB $Re$}%
\psfrag{029}[bc][bc]{\matlabtextB $F_{D,\phi=0^\circ}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $200$}%
\psfrag{002}[ct][ct]{\matlabtextC $400$}%
\psfrag{003}[ct][ct]{\matlabtextC $600$}%
\psfrag{004}[ct][ct]{\matlabtextC $800$}%
\psfrag{005}[ct][ct]{\matlabtextC $1000$}%
\psfrag{012}[ct][ct]{\matlabtextC $0$}%
\psfrag{013}[ct][ct]{\matlabtextC $200$}%
\psfrag{014}[ct][ct]{\matlabtextC $400$}%
\psfrag{015}[ct][ct]{\matlabtextC $600$}%
\psfrag{016}[ct][ct]{\matlabtextC $800$}%
\psfrag{017}[ct][ct]{\matlabtextC $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $50$}%
\psfrag{008}[rc][rc]{\matlabtextC $100$}%
\psfrag{009}[rc][rc]{\matlabtextC $150$}%
\psfrag{010}[rc][rc]{\matlabtextC $200$}%
\psfrag{011}[rc][rc]{\matlabtextC $250$}%
\psfrag{018}[rc][rc]{\matlabtextC $0$}%
\psfrag{019}[rc][rc]{\matlabtextC $50$}%
\psfrag{020}[rc][rc]{\matlabtextC $100$}%
\psfrag{021}[rc][rc]{\matlabtextC $150$}%
\psfrag{022}[rc][rc]{\matlabtextC $200$}%
\psfrag{023}[rc][rc]{\matlabtextC $250$}%
%
%% </ytick>

==> pics/Fd_vs_Re_loglog.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-20$10
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{018}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{021}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{019}[tc][tc]{\matlabtextB $Re$}%
\psfrag{020}[bc][bc]{\matlabtextB $F_{D,\phi=90^\circ}$}%
\psfrag{022}[tc][tc]{\matlabtextB $Re$}%
\psfrag{023}[bc][bc]{\matlabtextB $F_{D,\phi=0^\circ}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{-2}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{-1}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{0}$}%
\psfrag{003}[ct][ct]{\matlabtextC $10^{1}$}%
\psfrag{004}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{005}[ct][ct]{\matlabtextC $10^{3}$}%
\psfrag{009}[ct][ct]{\matlabtextC $10^{-2}$}%
\psfrag{010}[ct][ct]{\matlabtextC $10^{-1}$}%
\psfrag{011}[ct][ct]{\matlabtextC $10^{0}$}%
\psfrag{012}[ct][ct]{\matlabtextC $10^{1}$}%
\psfrag{013}[ct][ct]{\matlabtextC $10^{2}$}%
\psfrag{014}[ct][ct]{\matlabtextC $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $10^{0}$}%
\psfrag{007}[rc][rc]{\matlabtextC $10^{1}$}%
\psfrag{008}[rc][rc]{\matlabtextC $10^{2}$}%
\psfrag{015}[rc][rc]{\matlabtextC $10^{0}$}%
\psfrag{016}[rc][rc]{\matlabtextC $10^{1}$}%
\psfrag{017}[rc][rc]{\matlabtextC $10^{2}$}%
%
%% </ytick>

==> pics/FlVsReEps.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{062}[tl][tl]{\matlabtextA ($i$)}%
\psfrag{064}[tl][tl]{\matlabtextA ($f$)}%
\psfrag{065}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{066}[tl][tl]{\matlabtextA ($h$)}%
\psfrag{068}[tl][tl]{\matlabtextA ($e$)}%
\psfrag{069}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{070}[tl][tl]{\matlabtextA ($g$)}%
\psfrag{073}[tl][tl]{\matlabtextA ($d$)}%
\psfrag{075}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{063}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{067}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{071}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{072}[bc][bc]{\matlabtextB $F_L$}%
\psfrag{074}[bc][bc]{\matlabtextB $F_L$}%
\psfrag{076}[bc][bc]{\matlabtextB $F_L$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $15$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $45$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $75$}%
\psfrag{006}[ct][ct]{\matlabtextC $90$}%
\psfrag{021}[ct][ct]{\matlabtextC $0$}%
\psfrag{022}[ct][ct]{\matlabtextC $15$}%
\psfrag{023}[ct][ct]{\matlabtextC $30$}%
\psfrag{024}[ct][ct]{\matlabtextC $45$}%
\psfrag{025}[ct][ct]{\matlabtextC $60$}%
\psfrag{026}[ct][ct]{\matlabtextC $75$}%
\psfrag{027}[ct][ct]{\matlabtextC $90$}%
\psfrag{041}[ct][ct]{\matlabtextC $0$}%
\psfrag{042}[ct][ct]{\matlabtextC $15$}%
\psfrag{043}[ct][ct]{\matlabtextC $30$}%
\psfrag{044}[ct][ct]{\matlabtextC $45$}%
\psfrag{045}[ct][ct]{\matlabtextC $60$}%
\psfrag{046}[ct][ct]{\matlabtextC $75$}%
\psfrag{047}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $100$}%
\psfrag{009}[rc][rc]{\matlabtextC $200$}%
\psfrag{010}[rc][rc]{\matlabtextC $300$}%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $10$}%
\psfrag{013}[rc][rc]{\matlabtextC $20$}%
\psfrag{014}[rc][rc]{\matlabtextC $30$}%
\psfrag{015}[rc][rc]{\matlabtextC $40$}%
\psfrag{016}[rc][rc]{\matlabtextC $50$}%
\psfrag{017}[rc][rc]{\matlabtextC $0$}%
\psfrag{018}[rc][rc]{\matlabtextC $5$}%
\psfrag{019}[rc][rc]{\matlabtextC $10$}%
\psfrag{020}[rc][rc]{\matlabtextC $15$}%
\psfrag{028}[rc][rc]{\matlabtextC $0$}%
\psfrag{029}[rc][rc]{\matlabtextC $50$}%
\psfrag{030}[rc][rc]{\matlabtextC $100$}%
\psfrag{031}[rc][rc]{\matlabtextC $150$}%
\psfrag{032}[rc][rc]{\matlabtextC $0$}%
\psfrag{033}[rc][rc]{\matlabtextC $5$}%
\psfrag{034}[rc][rc]{\matlabtextC $10$}%
\psfrag{035}[rc][rc]{\matlabtextC $15$}%
\psfrag{036}[rc][rc]{\matlabtextC $0$}%
\psfrag{037}[rc][rc]{\matlabtextC $2$}%
\psfrag{038}[rc][rc]{\matlabtextC $4$}%
\psfrag{039}[rc][rc]{\matlabtextC $6$}%
\psfrag{040}[rc][rc]{\matlabtextC $8$}%
\psfrag{048}[rc][rc]{\matlabtextC $0$}%
\psfrag{049}[rc][rc]{\matlabtextC $20$}%
\psfrag{050}[rc][rc]{\matlabtextC $40$}%
\psfrag{051}[rc][rc]{\matlabtextC $60$}%
\psfrag{052}[rc][rc]{\matlabtextC $80$}%
\psfrag{053}[rc][rc]{\matlabtextC $0$}%
\psfrag{054}[rc][rc]{\matlabtextC $2$}%
\psfrag{055}[rc][rc]{\matlabtextC $4$}%
\psfrag{056}[rc][rc]{\matlabtextC $6$}%
\psfrag{057}[rc][rc]{\matlabtextC $8$}%
\psfrag{058}[rc][rc]{\matlabtextC $0$}%
\psfrag{059}[rc][rc]{\matlabtextC $1$}%
\psfrag{060}[rc][rc]{\matlabtextC $2$}%
\psfrag{061}[rc][rc]{\matlabtextC $3$}%
%
%% </ytick>

==> pics/Fl_Re100_eps0_3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextA $\phi[^\circ]$}%
\psfrag{014}[bc][bc]{\matlabtextA $F_L$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $15$}%
\psfrag{002}[ct][ct]{\matlabtextB $30$}%
\psfrag{003}[ct][ct]{\matlabtextB $45$}%
\psfrag{004}[ct][ct]{\matlabtextB $60$}%
\psfrag{005}[ct][ct]{\matlabtextB $75$}%
\psfrag{006}[ct][ct]{\matlabtextB $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $5$}%
\psfrag{009}[rc][rc]{\matlabtextB $10$}%
\psfrag{010}[rc][rc]{\matlabtextB $15$}%
\psfrag{011}[rc][rc]{\matlabtextB $20$}%
\psfrag{012}[rc][rc]{\matlabtextB $25$}%
%
%% </ytick>

==> pics/Flmax_vs_FdDiff.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{010}[tl][tl]{\matlabtextA $F_{D,\phi=90^\circ} - F_{D,\phi=0^\circ}$}%
\psfrag{011}[tl][tl]{\matlabtextA $F_{L,simple}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextB $\epsilon_s$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.4$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $50$}%
\psfrag{007}[rc][rc]{\matlabtextC $100$}%
\psfrag{008}[rc][rc]{\matlabtextC $150$}%
\psfrag{009}[rc][rc]{\matlabtextC $200$}%
%
%% </ytick>

==> pics/RegimeMap.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{011}[tc][tc]{\matlabtextA $Re$}%
\psfrag{012}[bc][bc]{\matlabtextA $\epsilon_s$}%

%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{-1}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{0}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{1}$}%
\psfrag{003}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{004}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $0$}%
\psfrag{006}[rc][rc]{\matlabtextB $0.1$}%
\psfrag{007}[rc][rc]{\matlabtextB $0.2$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.3$}%
\psfrag{009}[rc][rc]{\matlabtextB $0.4$}%
\psfrag{010}[rc][rc]{\matlabtextB $0.5$}%
%
%% </ytick>
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{7}{7}\selectfont\strut}%
\psfrag{013}[bc][bc]{\matlabtextC  }%
\psfrag{014}[bc][bc]{\matlabtextB Stokes \newline Regime}%
\psfrag{015}[bc][bc]{\matlabtextB \cite{sanjeevi2017orientational}}%

==> pics/StdDev_ReEps.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $\phi [^\circ]$}%
\psfrag{013}[bc][bc]{\matlabtextA $\sigma_{F_D}/F_D$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $15$}%
\psfrag{002}[ct][ct]{\matlabtextB $30$}%
\psfrag{003}[ct][ct]{\matlabtextB $45$}%
\psfrag{004}[ct][ct]{\matlabtextB $60$}%
\psfrag{005}[ct][ct]{\matlabtextB $75$}%
\psfrag{006}[ct][ct]{\matlabtextB $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0.2$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.4$}%
\psfrag{009}[rc][rc]{\matlabtextB $0.6$}%
\psfrag{010}[rc][rc]{\matlabtextB $0.8$}%
\psfrag{011}[rc][rc]{\matlabtextB $1$}%
%
%% </ytick>

==> pics/TpFit_vs_Re_loglog.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{006}[tc][tc]{\matlabtextA $Re$}%
\psfrag{007}[bc][bc]{\matlabtextA $T_{P,mag}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $10^{1}$}%
\psfrag{001}[ct][ct]{\matlabtextB $10^{2}$}%
\psfrag{002}[ct][ct]{\matlabtextB $10^{3}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{004}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{2}$}%
%
%% </ytick>

==> pics/TpVsReEps.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{048}[tl][tl]{\matlabtextA ($f$)}%
\psfrag{050}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{051}[tl][tl]{\matlabtextA ($e$)}%
\psfrag{053}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{054}[tl][tl]{\matlabtextA ($d$)}%
\psfrag{057}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{049}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{052}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{055}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{056}[bc][bc]{\matlabtextB $T_P$}%
\psfrag{058}[bc][bc]{\matlabtextB $T_P$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $15$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $45$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $75$}%
\psfrag{006}[ct][ct]{\matlabtextC $90$}%
\psfrag{017}[ct][ct]{\matlabtextC $0$}%
\psfrag{018}[ct][ct]{\matlabtextC $15$}%
\psfrag{019}[ct][ct]{\matlabtextC $30$}%
\psfrag{020}[ct][ct]{\matlabtextC $45$}%
\psfrag{021}[ct][ct]{\matlabtextC $60$}%
\psfrag{022}[ct][ct]{\matlabtextC $75$}%
\psfrag{023}[ct][ct]{\matlabtextC $90$}%
\psfrag{032}[ct][ct]{\matlabtextC $0$}%
\psfrag{033}[ct][ct]{\matlabtextC $15$}%
\psfrag{034}[ct][ct]{\matlabtextC $30$}%
\psfrag{035}[ct][ct]{\matlabtextC $45$}%
\psfrag{036}[ct][ct]{\matlabtextC $60$}%
\psfrag{037}[ct][ct]{\matlabtextC $75$}%
\psfrag{038}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $100$}%
\psfrag{009}[rc][rc]{\matlabtextC $200$}%
\psfrag{010}[rc][rc]{\matlabtextC $300$}%
\psfrag{011}[rc][rc]{\matlabtextC $400$}%
\psfrag{012}[rc][rc]{\matlabtextC $0$}%
\psfrag{013}[rc][rc]{\matlabtextC $20$}%
\psfrag{014}[rc][rc]{\matlabtextC $40$}%
\psfrag{015}[rc][rc]{\matlabtextC $60$}%
\psfrag{016}[rc][rc]{\matlabtextC $80$}%
\psfrag{024}[rc][rc]{\matlabtextC $0$}%
\psfrag{025}[rc][rc]{\matlabtextC $50$}%
\psfrag{026}[rc][rc]{\matlabtextC $100$}%
\psfrag{027}[rc][rc]{\matlabtextC $150$}%
\psfrag{028}[rc][rc]{\matlabtextC $0$}%
\psfrag{029}[rc][rc]{\matlabtextC $10$}%
\psfrag{030}[rc][rc]{\matlabtextC $20$}%
\psfrag{031}[rc][rc]{\matlabtextC $30$}%
\psfrag{039}[rc][rc]{\matlabtextC $0$}%
\psfrag{040}[rc][rc]{\matlabtextC $20$}%
\psfrag{041}[rc][rc]{\matlabtextC $40$}%
\psfrag{042}[rc][rc]{\matlabtextC $60$}%
\psfrag{043}[rc][rc]{\matlabtextC $80$}%
\psfrag{044}[rc][rc]{\matlabtextC $0$}%
\psfrag{045}[rc][rc]{\matlabtextC $5$}%
\psfrag{046}[rc][rc]{\matlabtextC $10$}%
\psfrag{047}[rc][rc]{\matlabtextC $15$}%
%
%% </ytick>

==> pics/axVelHist.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{018}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{019}[tl][tl]{\matlabtextA ($d$)}%
\psfrag{021}[tl][tl]{\matlabtextA ($a$)}%
\psfrag{023}[tl][tl]{\matlabtextA ($c$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{020}[tc][tc]{\matlabtextB $u_{ax}/u_{avg}$}%
\psfrag{022}[bc][bc]{\matlabtextB Probability}%
\psfrag{024}[tc][tc]{\matlabtextB $u_{ax}/u_{avg}$}%
\psfrag{025}[bc][bc]{\matlabtextB Probability}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $1$}%
\psfrag{002}[ct][ct]{\matlabtextC $2$}%
\psfrag{003}[ct][ct]{\matlabtextC $3$}%
\psfrag{004}[ct][ct]{\matlabtextC $4$}%
\psfrag{009}[ct][ct]{\matlabtextC $0$}%
\psfrag{010}[ct][ct]{\matlabtextC $1$}%
\psfrag{011}[ct][ct]{\matlabtextC $2$}%
\psfrag{012}[ct][ct]{\matlabtextC $3$}%
\psfrag{013}[ct][ct]{\matlabtextC $4$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextC $0$}%
\psfrag{006}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.15$}%
\psfrag{014}[rc][rc]{\matlabtextC $0$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.15$}%
%
%% </ytick>

==> pics/comsol_vs_lb3d.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{013}[tc][tc]{\matlabtextA $\phi[^\circ]$}%
\psfrag{014}[bc][bc]{\matlabtextA $F_D$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $15$}%
\psfrag{002}[ct][ct]{\matlabtextB $30$}%
\psfrag{003}[ct][ct]{\matlabtextB $45$}%
\psfrag{004}[ct][ct]{\matlabtextB $60$}%
\psfrag{005}[ct][ct]{\matlabtextB $75$}%
\psfrag{006}[ct][ct]{\matlabtextB $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $10$}%
\psfrag{009}[rc][rc]{\matlabtextB $20$}%
\psfrag{010}[rc][rc]{\matlabtextB $30$}%
\psfrag{011}[rc][rc]{\matlabtextB $40$}%
\psfrag{012}[rc][rc]{\matlabtextB $50$}%
%
%% </ytick>

==> pics/configVelHist.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{018}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{019}[tl][tl]{\matlabtextA ($a$)}%
\psfrag{021}[tl][tl]{\matlabtextA ($d$)}%
\psfrag{023}[tl][tl]{\matlabtextA ($c$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB Probability}%
\psfrag{022}[tc][tc]{\matlabtextB $u_{ax}/u_{avg}$}%
\psfrag{024}[tc][tc]{\matlabtextB $u_{ax}/u_{avg}$}%
\psfrag{025}[bc][bc]{\matlabtextB Probability}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{004}[ct][ct]{\matlabtextC $0$}%
\psfrag{005}[ct][ct]{\matlabtextC $1$}%
\psfrag{006}[ct][ct]{\matlabtextC $2$}%
\psfrag{007}[ct][ct]{\matlabtextC $3$}%
\psfrag{008}[ct][ct]{\matlabtextC $4$}%
\psfrag{009}[ct][ct]{\matlabtextC $0$}%
\psfrag{010}[ct][ct]{\matlabtextC $1$}%
\psfrag{011}[ct][ct]{\matlabtextC $2$}%
\psfrag{012}[ct][ct]{\matlabtextC $3$}%
\psfrag{013}[ct][ct]{\matlabtextC $4$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[rc][rc]{\matlabtextC $0$}%
\psfrag{001}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{002}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{003}[rc][rc]{\matlabtextC $0.15$}%
\psfrag{014}[rc][rc]{\matlabtextC $0$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.05$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{017}[rc][rc]{\matlabtextC $0.15$}%
%
%% </ytick>

==> pics/config_subplot.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{033}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{034}[tl][tl]{\matlabtextA ($f$)}%
\psfrag{036}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{037}[tl][tl]{\matlabtextA ($e$)}%
\psfrag{039}[tl][tl]{\matlabtextA ($a$)}%
\psfrag{041}[tl][tl]{\matlabtextA ($d$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{035}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{038}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{040}[bc][bc]{\matlabtextB $F_D$}%
\psfrag{042}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{043}[bc][bc]{\matlabtextB $F_D$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $15$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $45$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $75$}%
\psfrag{006}[ct][ct]{\matlabtextC $90$}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $15$}%
\psfrag{009}[ct][ct]{\matlabtextC $30$}%
\psfrag{010}[ct][ct]{\matlabtextC $45$}%
\psfrag{011}[ct][ct]{\matlabtextC $60$}%
\psfrag{012}[ct][ct]{\matlabtextC $75$}%
\psfrag{013}[ct][ct]{\matlabtextC $90$}%
\psfrag{020}[ct][ct]{\matlabtextC $0$}%
\psfrag{021}[ct][ct]{\matlabtextC $15$}%
\psfrag{022}[ct][ct]{\matlabtextC $30$}%
\psfrag{023}[ct][ct]{\matlabtextC $45$}%
\psfrag{024}[ct][ct]{\matlabtextC $60$}%
\psfrag{025}[ct][ct]{\matlabtextC $75$}%
\psfrag{026}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{014}[rc][rc]{\matlabtextC $0$}%
\psfrag{015}[rc][rc]{\matlabtextC $10$}%
\psfrag{016}[rc][rc]{\matlabtextC $20$}%
\psfrag{017}[rc][rc]{\matlabtextC $30$}%
\psfrag{018}[rc][rc]{\matlabtextC $40$}%
\psfrag{019}[rc][rc]{\matlabtextC $50$}%
\psfrag{027}[rc][rc]{\matlabtextC $0$}%
\psfrag{028}[rc][rc]{\matlabtextC $10$}%
\psfrag{029}[rc][rc]{\matlabtextC $20$}%
\psfrag{030}[rc][rc]{\matlabtextC $30$}%
\psfrag{031}[rc][rc]{\matlabtextC $40$}%
\psfrag{032}[rc][rc]{\matlabtextC $50$}%
%
%% </ytick>

==> pics/configs_hist.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{028}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{029}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{030}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{031}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{032}[bc][bc]{\matlabtextB Number of particles}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $15$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $45$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $75$}%
\psfrag{006}[ct][ct]{\matlabtextC $90$}%
\psfrag{014}[ct][ct]{\matlabtextC $0$}%
\psfrag{015}[ct][ct]{\matlabtextC $15$}%
\psfrag{016}[ct][ct]{\matlabtextC $30$}%
\psfrag{017}[ct][ct]{\matlabtextC $45$}%
\psfrag{018}[ct][ct]{\matlabtextC $60$}%
\psfrag{019}[ct][ct]{\matlabtextC $75$}%
\psfrag{020}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $20$}%
\psfrag{009}[rc][rc]{\matlabtextC $40$}%
\psfrag{010}[rc][rc]{\matlabtextC $60$}%
\psfrag{011}[rc][rc]{\matlabtextC $80$}%
\psfrag{012}[rc][rc]{\matlabtextC $100$}%
\psfrag{013}[rc][rc]{\matlabtextC $120$}%
\psfrag{021}[rc][rc]{\matlabtextC $0$}%
\psfrag{022}[rc][rc]{\matlabtextC $20$}%
\psfrag{023}[rc][rc]{\matlabtextC $40$}%
\psfrag{024}[rc][rc]{\matlabtextC $60$}%
\psfrag{025}[rc][rc]{\matlabtextC $80$}%
\psfrag{026}[rc][rc]{\matlabtextC $100$}%
\psfrag{027}[rc][rc]{\matlabtextC $120$}%
%
%% </ytick>

==> pics/dragRatios.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $\epsilon_s$}%
\psfrag{013}[bc][bc]{\matlabtextA $F_{D,\phi=90^\circ}/F_{D,\phi=0^\circ}$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{005}[ct][ct]{\matlabtextB $0.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $1$}%
\psfrag{007}[rc][rc]{\matlabtextB $2$}%
\psfrag{008}[rc][rc]{\matlabtextB $3$}%
\psfrag{009}[rc][rc]{\matlabtextB $4$}%
\psfrag{010}[rc][rc]{\matlabtextB $5$}%
\psfrag{011}[rc][rc]{\matlabtextB $6$}%
%
%% </ytick>

==> pics/eps0_1_config_independence.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{039}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{040}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{041}[tl][tl]{\matlabtextA ($a$)}%
\psfrag{043}[tl][tl]{\matlabtextA ($f$)}%
\psfrag{044}[tl][tl]{\matlabtextA ($e$)}%
\psfrag{045}[tl][tl]{\matlabtextA ($d$)}%
\psfrag{047}[tl][tl]{\matlabtextA ($i$)}%
\psfrag{049}[tl][tl]{\matlabtextA ($h$)}%
\psfrag{051}[tl][tl]{\matlabtextA ($g$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{042}[bc][bc]{\matlabtextB $F_D$}%
\psfrag{046}[bc][bc]{\matlabtextB $F_D$}%
\psfrag{048}[tc][tc]{\matlabtextB $\phi$}%
\psfrag{050}[tc][tc]{\matlabtextB $\phi$}%
\psfrag{052}[tc][tc]{\matlabtextB $\phi$}%
\psfrag{053}[bc][bc]{\matlabtextB $F_D$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{012}[ct][ct]{\matlabtextC $0$}%
\psfrag{013}[ct][ct]{\matlabtextC $15$}%
\psfrag{014}[ct][ct]{\matlabtextC $30$}%
\psfrag{015}[ct][ct]{\matlabtextC $45$}%
\psfrag{016}[ct][ct]{\matlabtextC $60$}%
\psfrag{017}[ct][ct]{\matlabtextC $75$}%
\psfrag{018}[ct][ct]{\matlabtextC $90$}%
\psfrag{019}[ct][ct]{\matlabtextC $0$}%
\psfrag{020}[ct][ct]{\matlabtextC $15$}%
\psfrag{021}[ct][ct]{\matlabtextC $30$}%
\psfrag{022}[ct][ct]{\matlabtextC $45$}%
\psfrag{023}[ct][ct]{\matlabtextC $60$}%
\psfrag{024}[ct][ct]{\matlabtextC $75$}%
\psfrag{025}[ct][ct]{\matlabtextC $90$}%
\psfrag{026}[ct][ct]{\matlabtextC $0$}%
\psfrag{027}[ct][ct]{\matlabtextC $15$}%
\psfrag{028}[ct][ct]{\matlabtextC $30$}%
\psfrag{029}[ct][ct]{\matlabtextC $45$}%
\psfrag{030}[ct][ct]{\matlabtextC $60$}%
\psfrag{031}[ct][ct]{\matlabtextC $75$}%
\psfrag{032}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[rc][rc]{\matlabtextC $1$}%
\psfrag{001}[rc][rc]{\matlabtextC $1.5$}%
\psfrag{002}[rc][rc]{\matlabtextC $2$}%
\psfrag{003}[rc][rc]{\matlabtextC $2.5$}%
\psfrag{004}[rc][rc]{\matlabtextC $3$}%
\psfrag{005}[rc][rc]{\matlabtextC $3.5$}%
\psfrag{006}[rc][rc]{\matlabtextC $4$}%
\psfrag{007}[rc][rc]{\matlabtextC $4.5$}%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $5$}%
\psfrag{010}[rc][rc]{\matlabtextC $10$}%
\psfrag{011}[rc][rc]{\matlabtextC $15$}%
\psfrag{033}[rc][rc]{\matlabtextC $0$}%
\psfrag{034}[rc][rc]{\matlabtextC $20$}%
\psfrag{035}[rc][rc]{\matlabtextC $40$}%
\psfrag{036}[rc][rc]{\matlabtextC $60$}%
\psfrag{037}[rc][rc]{\matlabtextC $80$}%
\psfrag{038}[rc][rc]{\matlabtextC $100$}%
%
%% </ytick>

==> pics/eps0_3_config_independence.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{035}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{036}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{037}[tl][tl]{\matlabtextA ($a$)}%
\psfrag{039}[tl][tl]{\matlabtextA ($f$)}%
\psfrag{041}[tl][tl]{\matlabtextA ($e$)}%
\psfrag{043}[tl][tl]{\matlabtextA ($d$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{038}[bc][bc]{\matlabtextB $F_D$}%
\psfrag{040}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{042}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{044}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{045}[bc][bc]{\matlabtextB $F_D$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $15$}%
\psfrag{009}[ct][ct]{\matlabtextC $30$}%
\psfrag{010}[ct][ct]{\matlabtextC $45$}%
\psfrag{011}[ct][ct]{\matlabtextC $60$}%
\psfrag{012}[ct][ct]{\matlabtextC $75$}%
\psfrag{013}[ct][ct]{\matlabtextC $90$}%
\psfrag{014}[ct][ct]{\matlabtextC $0$}%
\psfrag{015}[ct][ct]{\matlabtextC $15$}%
\psfrag{016}[ct][ct]{\matlabtextC $30$}%
\psfrag{017}[ct][ct]{\matlabtextC $45$}%
\psfrag{018}[ct][ct]{\matlabtextC $60$}%
\psfrag{019}[ct][ct]{\matlabtextC $75$}%
\psfrag{020}[ct][ct]{\matlabtextC $90$}%
\psfrag{021}[ct][ct]{\matlabtextC $0$}%
\psfrag{022}[ct][ct]{\matlabtextC $15$}%
\psfrag{023}[ct][ct]{\matlabtextC $30$}%
\psfrag{024}[ct][ct]{\matlabtextC $45$}%
\psfrag{025}[ct][ct]{\matlabtextC $60$}%
\psfrag{026}[ct][ct]{\matlabtextC $75$}%
\psfrag{027}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{000}[rc][rc]{\matlabtextC $6$}%
\psfrag{001}[rc][rc]{\matlabtextC $8$}%
\psfrag{002}[rc][rc]{\matlabtextC $10$}%
\psfrag{003}[rc][rc]{\matlabtextC $12$}%
\psfrag{004}[rc][rc]{\matlabtextC $14$}%
\psfrag{005}[rc][rc]{\matlabtextC $16$}%
\psfrag{006}[rc][rc]{\matlabtextC $18$}%
\psfrag{028}[rc][rc]{\matlabtextC $0$}%
\psfrag{029}[rc][rc]{\matlabtextC $50$}%
\psfrag{030}[rc][rc]{\matlabtextC $100$}%
\psfrag{031}[rc][rc]{\matlabtextC $150$}%
\psfrag{032}[rc][rc]{\matlabtextC $200$}%
\psfrag{033}[rc][rc]{\matlabtextC $250$}%
\psfrag{034}[rc][rc]{\matlabtextC $300$}%
%
%% </ytick>

==> pics/eps0_5_config_independence.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{029}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{031}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{033}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{030}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{032}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{034}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{035}[bc][bc]{\matlabtextB $F_D$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $15$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $45$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $75$}%
\psfrag{006}[ct][ct]{\matlabtextC $90$}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $15$}%
\psfrag{009}[ct][ct]{\matlabtextC $30$}%
\psfrag{010}[ct][ct]{\matlabtextC $45$}%
\psfrag{011}[ct][ct]{\matlabtextC $60$}%
\psfrag{012}[ct][ct]{\matlabtextC $75$}%
\psfrag{013}[ct][ct]{\matlabtextC $90$}%
\psfrag{014}[ct][ct]{\matlabtextC $0$}%
\psfrag{015}[ct][ct]{\matlabtextC $15$}%
\psfrag{016}[ct][ct]{\matlabtextC $30$}%
\psfrag{017}[ct][ct]{\matlabtextC $45$}%
\psfrag{018}[ct][ct]{\matlabtextC $60$}%
\psfrag{019}[ct][ct]{\matlabtextC $75$}%
\psfrag{020}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{021}[rc][rc]{\matlabtextC $0$}%
\psfrag{022}[rc][rc]{\matlabtextC $20$}%
\psfrag{023}[rc][rc]{\matlabtextC $40$}%
\psfrag{024}[rc][rc]{\matlabtextC $60$}%
\psfrag{025}[rc][rc]{\matlabtextC $80$}%
\psfrag{026}[rc][rc]{\matlabtextC $100$}%
\psfrag{027}[rc][rc]{\matlabtextC $120$}%
\psfrag{028}[rc][rc]{\matlabtextC $140$}%
%
%% </ytick>

==> pics/flowvec.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{001}[tl][tl]{\matlabtextB $\hat{\bm{e}}_1$ ($\bm{u}_s$ and $\bm{F}_D$ direction)}%
\psfrag{002}[tl][tl]{\matlabtextB $\hat{\bm{e}}_2$}%
\psfrag{003}[tl][tl]{\matlabtextB $\hat{\bm{e}}_3$ ($\bm{F}_L$ direction)}%
\psfrag{004}[tc][tc]{\matlabtextB $\bm{p}$}%
\psfrag{005}[tc][tc]{\matlabtextB $\phi$}%
\psfrag{007}[tc][tc]{\matlabtextB $\bm{T}_P$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{10}{10}\selectfont\strut}%
\psfrag{006}[tl][tl]{\matlabtextC \text{Plane contains $\hat{\bm{e}}_1$, $\hat{\bm{e}}_3$, and $\bm{p}$}}%
%\psfrag{007}[tc][tc]{\matlabtextC \text{drag}}%
%\psfrag{008}[bc][bc]{\matlabtextC \emph{lift}}%


%
%% </xtick>
%
%% <ytick>
%

%
%% </ytick>

==> pics/lateral_force_independence.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{016}[tc][tc]{\matlabtextA $\phi[^\circ]$}%
\psfrag{017}[bc][bc]{\matlabtextA $F_2$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $15$}%
\psfrag{002}[ct][ct]{\matlabtextB $30$}%
\psfrag{003}[ct][ct]{\matlabtextB $45$}%
\psfrag{004}[ct][ct]{\matlabtextB $60$}%
\psfrag{005}[ct][ct]{\matlabtextB $75$}%
\psfrag{006}[ct][ct]{\matlabtextB $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $-40$}%
\psfrag{008}[rc][rc]{\matlabtextB $-30$}%
\psfrag{009}[rc][rc]{\matlabtextB $-20$}%
\psfrag{010}[rc][rc]{\matlabtextB $-10$}%
\psfrag{011}[rc][rc]{\matlabtextB $0$}%
\psfrag{012}[rc][rc]{\matlabtextB $10$}%
\psfrag{013}[rc][rc]{\matlabtextB $20$}%
\psfrag{014}[rc][rc]{\matlabtextB $30$}%
\psfrag{015}[rc][rc]{\matlabtextB $40$}%
%
%% </ytick>

==> pics/liftDragRatios.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{021}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{022}[tl][tl]{\matlabtextA ($d$)}%
\psfrag{023}[tl][tl]{\matlabtextA ($f$)}%
\psfrag{025}[tl][tl]{\matlabtextA ($a$)}%
\psfrag{027}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{029}[tl][tl]{\matlabtextA ($e$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{024}[tc][tc]{\matlabtextB $|F_L|/F_D$}%
\psfrag{026}[bc][bc]{\matlabtextB Probability}%
\psfrag{028}[bc][bc]{\matlabtextB Probability}%
\psfrag{030}[tc][tc]{\matlabtextB $|F_L|/F_D$}%
\psfrag{031}[bc][bc]{\matlabtextB Probability}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{005}[ct][ct]{\matlabtextC $1$}%
\psfrag{012}[ct][ct]{\matlabtextC $0$}%
\psfrag{013}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{014}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{015}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{016}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{017}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $0$}%
\psfrag{007}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{009}[rc][rc]{\matlabtextC $0$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{018}[rc][rc]{\matlabtextC $0$}%
\psfrag{019}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{020}[rc][rc]{\matlabtextC $0.4$}%
%
%% </ytick>

==> pics/nonsph_configs.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
%\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
%\psfrag{001}[tc][tc]{\matlabtextA Random}%
%\psfrag{002}[tc][tc]{\matlabtextA Planar random}%
%\psfrag{003}[tc][tc]{\matlabtextA Unidirectional}%
%%
%% </text>
%
% <xtick>

\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{001}[ct][ct]{\matlabtextB ($a$)}%
\psfrag{002}[ct][ct]{\matlabtextB ($b$)}%
\psfrag{003}[ct][ct]{\matlabtextB ($c$)}%

%%
%%% </xtick>
%%
%%% <ytick>
%%
%\psfrag{005}[rc][rc]{\matlabtextB $1$}%
%\psfrag{006}[rc][rc]{\matlabtextB $1.05$}%
%\psfrag{007}[rc][rc]{\matlabtextB $1.1$}%
%\psfrag{008}[rc][rc]{\matlabtextB $1.15$}%
%\psfrag{009}[rc][rc]{\matlabtextB $1.2$}%
%%
%%% </ytick>

==> pics/orientation.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
%\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
%\psfrag{001}[tc][tc]{\matlabtextA Random}%
%\psfrag{002}[tc][tc]{\matlabtextA Planar random}%
%\psfrag{003}[tc][tc]{\matlabtextA Unidirectional}%
%
%% </text>
%
% <xtick>

\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{001}[ct][ct]{\matlabtextB ($a$)}%
\psfrag{002}[ct][ct]{\matlabtextB ($b$)}%
\psfrag{003}[ct][ct]{\matlabtextB ($c$)}%

\psfrag{004}[ct][ct]{\matlabtextB $x$}%
\psfrag{005}[ct][ct]{\matlabtextB $y$}%
\psfrag{006}[ct][ct]{\matlabtextB $z$}%
%%
%%% </xtick>
%%
%%% <ytick>
%%
%\psfrag{005}[rc][rc]{\matlabtextB $1$}%
%\psfrag{006}[rc][rc]{\matlabtextB $1.05$}%
%\psfrag{007}[rc][rc]{\matlabtextB $1.1$}%
%\psfrag{008}[rc][rc]{\matlabtextB $1.15$}%
%\psfrag{009}[rc][rc]{\matlabtextB $1.2$}%
%%
%%% </ytick>

==> pics/packedHistogram.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $\phi[^\circ]$}%
\psfrag{013}[bc][bc]{\matlabtextA Probability}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $15$}%
\psfrag{002}[ct][ct]{\matlabtextB $30$}%
\psfrag{003}[ct][ct]{\matlabtextB $45$}%
\psfrag{004}[ct][ct]{\matlabtextB $60$}%
\psfrag{005}[ct][ct]{\matlabtextB $75$}%
\psfrag{006}[ct][ct]{\matlabtextB $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextB $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextB $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextB $0.4$}%
%
%% </ytick>

==> pics/stream_lines.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
%\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
%\psfrag{001}[tc][tc]{\matlabtextA Random}%
%\psfrag{002}[tc][tc]{\matlabtextA Planar random}%
%\psfrag{003}[tc][tc]{\matlabtextA Unidirectional}%
%
%% </text>
%
% <xtick>

\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB 0}%
\psfrag{001}[ct][ct]{\matlabtextB 1.5}%
\psfrag{002}[ct][ct]{\matlabtextB 3.0}%
\psfrag{003}[ct][ct]{\matlabtextB 4.5}%

\psfrag{004}[ct][ct]{\matlabtextB $x$}%
\psfrag{005}[ct][ct]{\matlabtextB $y$}%
\psfrag{006}[ct][ct]{\matlabtextB $z$}%

\psfrag{007}[ct][ct]{\matlabtextB $|\bm{u}|/|\bm{u}_s|$}%

%%
%%% </xtick>
%%
%%% <ytick>
%%
%\psfrag{005}[rc][rc]{\matlabtextB $1$}%
%\psfrag{006}[rc][rc]{\matlabtextB $1.05$}%
%\psfrag{007}[rc][rc]{\matlabtextB $1.1$}%
%\psfrag{008}[rc][rc]{\matlabtextB $1.15$}%
%\psfrag{009}[rc][rc]{\matlabtextB $1.2$}%
%%
%%% </ytick>

==> pics/torque_independence.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{025}[tl][tl]{\matlabtextA ($c$)}%
\psfrag{028}[tl][tl]{\matlabtextA ($b$)}%
\psfrag{031}[tl][tl]{\matlabtextA ($a$)}%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{9}{9}\selectfont\strut}%
\psfrag{026}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{027}[bc][bc]{\matlabtextB $T_3$}%
\psfrag{029}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{030}[bc][bc]{\matlabtextB $T_2$}%
\psfrag{032}[tc][tc]{\matlabtextB $\phi[^\circ]$}%
\psfrag{033}[bc][bc]{\matlabtextB $T_1$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $15$}%
\psfrag{002}[ct][ct]{\matlabtextC $30$}%
\psfrag{003}[ct][ct]{\matlabtextC $45$}%
\psfrag{004}[ct][ct]{\matlabtextC $60$}%
\psfrag{005}[ct][ct]{\matlabtextC $75$}%
\psfrag{006}[ct][ct]{\matlabtextC $90$}%
\psfrag{007}[ct][ct]{\matlabtextC $0$}%
\psfrag{008}[ct][ct]{\matlabtextC $15$}%
\psfrag{009}[ct][ct]{\matlabtextC $30$}%
\psfrag{010}[ct][ct]{\matlabtextC $45$}%
\psfrag{011}[ct][ct]{\matlabtextC $60$}%
\psfrag{012}[ct][ct]{\matlabtextC $75$}%
\psfrag{013}[ct][ct]{\matlabtextC $90$}%
\psfrag{014}[ct][ct]{\matlabtextC $0$}%
\psfrag{015}[ct][ct]{\matlabtextC $15$}%
\psfrag{016}[ct][ct]{\matlabtextC $30$}%
\psfrag{017}[ct][ct]{\matlabtextC $45$}%
\psfrag{018}[ct][ct]{\matlabtextC $60$}%
\psfrag{019}[ct][ct]{\matlabtextC $75$}%
\psfrag{020}[ct][ct]{\matlabtextC $90$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{021}[rc][rc]{\matlabtextC $-10$}%
\psfrag{022}[rc][rc]{\matlabtextC $0$}%
\psfrag{023}[rc][rc]{\matlabtextC $10$}%
\psfrag{024}[rc][rc]{\matlabtextC $20$}%
%
%% </ytick>
